A Magneto-Optical Trap of Titanium Atoms

We realize laser cooling and trapping of titanium (Ti) atoms in a mangeto-optical trap (MOT). While Ti does not possess a transition suitable for laser cooling out of its $\mathrm{3d^24s^2}$ $\mathrm{a^3F}$ ground term, there is such a transition, at an optical wavelength of $\lambda=498\mathrm{nm}$, from the long-lived $\mathrm{3d^3(^4F)4s}$ $\mathrm{a^5F_5}$ metastable state to the $\mathrm{3d^3(^4F)4p}$ $\mathrm{y^5G^o_6}$ excited state. Without the addition of any repumping light, we observe MOTs of metastable $\mathrm{^{46}Ti}$, $\mathrm{^{48}Ti}$, and $\mathrm{^{50}Ti}$, the three stable nuclear-spin-zero bosonic isotopes of Ti. While MOTs can be observed when loaded directly from our Ti sublimation source, optical pumping of ground term atoms to the $\mathrm{a^5F_5}$ state increases the loading rate by a factor of 120, and the steady-state MOT atom number by a factor of 30. At steady state, the MOT of $\mathrm{^{48}Ti}$ holds up to $8.30(26)\times10^5$ atoms at a maximum density of $1.3(4)\times10^{11}\mathrm{cm}^{-3}$ and at a temperature of $90(15)\mathrm{\mu K}$. By measuring the decay of the MOT upon suddenly reducing the loading rate, we place upper bounds on the leakage branching ratio of the cooling transition $(\leq2.5\times 10^{-6})$ and the two-body loss coefficient $(\leq2\times10^{-10}\mathrm{cm}^3\mathrm{s}^{-1})$. Our approach to laser cooling Ti can be applied to other transition metals, enabling a significant expansion of the elements that can be laser cooled.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
